Deep Network Flow for Multi-Object Tracking

Data association problems are an important component of many computer vision applications, with multi-object tracking being one of the most prominent examples. A typical approach to data association involves finding a graph matching or network flow that minimizes a sum of pairwise association costs, which are often either hand-crafted or learned as linear functions of fixed features. In this work, we demonstrate that it is possible to learn features for network-flow-based data association via backpropagation, by expressing the optimum of a smoothed network flow problem as a differentiable function of the pairwise association costs. We apply this approach to multi-object tracking with a network flow formulation. Our experiments demonstrate that we are able to successfully learn all cost functions for the association problem in an end-to-end fashion, which outperform hand-crafted costs in all settings. The integration and combination of various sources of inputs becomes easy and the cost functions can be learned entirely from data, alleviating tedious hand-designing of costs.

==> figures/loss/inputs_motion_train.tex <==
%!TEX root = ../deep_network_flow_cvpr17.tex
\begin{tikzpicture}\scriptsize
% http://tex.stackexchange.com/questions/42697/pgfplots-legends-in-multiple-y-axis-plot-overlapping

\pgfplotsset{
    scale only axis,
    xtick={0,1,2,3,4,5},
    xticklabels={0, 10k, 20k, 30k, 40k, 50k},
    xmin=0, xmax=5,
    y axis style/.style={
        yticklabel style=#1,
        ylabel style=#1,
        y axis line style=#1,
        ytick style=#1
   }
}

\begin{axis}[
  axis y line*=left,
  %y axis style=blue!75!black,
  ymin=0, ymax=15,
  %xlabel=iter,
  ylabel=loss
]
\addplot[blue,dashed,thick]
  coordinates{
    (0.0, 17.05128288)
    (0.5,  2.23264146)
    (1.0,  2.16148806)
    (1.5,  2.09548974)
    (2.0,  2.07985735)
    (2.5,  2.08121538)
    (3.0,  2.06464458)
    (3.5,  2.06113291)
    (4.0,  2.05237341)
    (4.5,  2.04711080)
    (5.0,  2.04823279)
};% (L) B+O+M
\addplot[red,dashed,thick]
  coordinates{
    (0.0, 16.98878098)
    (0.5,  2.35300422)
    (1.0,  2.30189657)
    (1.5,  2.22105908)
    (2.0,  2.27233291)
    (2.5,  2.21584344)
    (3.0,  2.20395780)
    (3.5,  2.15632319)
    (4.0,  2.16755724)
    (4.5,  2.17093277)
    (5.0,  2.16710973)
};% (L) B+O
\end{axis}

\begin{axis}[
  axis y line*=right,
  axis x line=none,
  ymin=0, ymax=1,
  ylabel=precision,
  %y axis style=red!75!black
]
\addplot[blue,solid,thick]
  coordinates{
    (0.0, 0.60255564)
    (0.5, 0.95528009)
    (1.0, 0.95795108)
    (1.5, 0.95949254)
    (2.0, 0.95994751)
    (2.5, 0.95976147)
    (3.0, 0.95987563)
    (3.5, 0.95995203)
    (4.0, 0.96055365)
    (4.5, 0.96062313)
    (5.0, 0.96064388)
};
\addplot[red,solid,thick]
  coordinates{
    (0.0, 0.60338817)
    (0.5, 0.95242921)
    (1.0, 0.95444199)
    (1.5, 0.95696441)
    (2.0, 0.95394126)
    (2.5, 0.95606558)
    (3.0, 0.95614196)
    (3.5, 0.95696254)
    (4.0, 0.95816041)
    (4.5, 0.95813469)
    (5.0, 0.95822958)
};
\end{axis}

\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../deep_network_flow_cvpr17"
%%% End:


==> figures/loss/inputs_motion_val.tex <==
%!TEX root = ../deep_network_flow_cvpr17.tex
\begin{tikzpicture}\scriptsize
% http://tex.stackexchange.com/questions/42697/pgfplots-legends-in-multiple-y-axis-plot-overlapping

\pgfplotsset{
    scale only axis,
    xtick={0,1,2,3,4,5},
    xticklabels={0, 10k, 20k, 30k, 40k, 50k},
    xmin=0, xmax=5,
    y axis style/.style={
        yticklabel style=#1,
        ylabel style=#1,
        y axis line style=#1,
        ytick style=#1
   }
}



\begin{axis}[
  axis y line*=left,
  %y axis style=blue!75!black,
  ymin=0, ymax=15,
  %xlabel=iter,
  ylabel=loss
  ]
\addplot[blue,dashed,thick]
  coordinates{
    (0.0, 15.79168034)
    (0.5,  1.61563981)
    (1.0,  1.46553147)
    (1.5,  1.37956846)
    (2.0,  1.34946215)
    (2.5,  1.38644826)
    (3.0,  1.34722269)
    (3.5,  1.34232807)
    (4.0,  1.37773836)
    (4.5,  1.40091288)
    (5.0,  1.40587330)
  };% (L) B+O+M
\addplot[red,dashed,thick]
  coordinates{
    (0.0, 15.71411419)
    (0.5,  1.59854090)
    (1.0,  1.55371034)
    (1.5,  1.47442448)
    (2.0,  1.42890823)
    (2.5,  1.40036881)
    (3.0,  1.40338469)
    (3.5,  1.35170424)
    (4.0,  1.40745270)
    (4.5,  1.40195608)
    (5.0,  1.45306718)
};% (L) B+O
\end{axis}

\begin{axis}[
  axis y line*=right,
  axis x line=none,
  ymin=0, ymax=1,
  ylabel=precision,
  %y axis style=red!75!black
  ]
\addplot[blue,solid,thick]
  coordinates{
    (0.0, 0.60476586)
    (0.5, 0.95355826)
    (1.0, 0.95691976)
    (1.5, 0.96507801)
    (2.0, 0.96345173)
    (2.5, 0.96340857)
    (3.0, 0.96400708)
    (3.5, 0.96390020)
    (4.0, 0.96325280)
    (4.5, 0.96290844)
    (5.0, 0.96288509)
  };
\addplot[red,solid,thick]
  coordinates{
    (0.0, 0.60500245)
    (0.5, 0.96329070)
    (1.0, 0.96413167)
    (1.5, 0.96514969)
    (2.0, 0.96363728)
    (2.5, 0.97110358)
    (3.0, 0.97084431)
    (3.5, 0.96663621)
    (4.0, 0.97028106)
    (4.5, 0.97044702)
    (5.0, 0.96969474)
};
\end{axis}

\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../deep_network_flow_cvpr17"
%%% End:


==> figures/tracker_model_nearonline.tex <==
%!TEX root = ../egpaper_for_review_suppmat.tex
\begin{tikzpicture}\footnotesize

\definecolor{temporalwindowcolor}{RGB}{90, 90, 90}
\definecolor{outputboxcolor}{RGB}{122, 61, 226}
\definecolor{incomingframeboxcolor}{RGB}{0, 150, 250}


\definecolor{trajectory1color}{RGB}{23, 120, 207}
\definecolor{trajectory2color}{RGB}{222, 16, 17}
\definecolor{trajectory3color}{RGB}{16, 222, 17}

%222, 16, 150

% ============================================================
% Detections over 8 frames
% ============================================================
\begin{scope}[shift={(0.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d11) at (0,0.00) {};
    \node (d12) at (0,0.60) {};
\end{scope}

\begin{scope}[shift={(1.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d21) at (0,0.00) {};
    \node (d22) at (0,0.70) {};
    \node (d23) at (0,1.40) {};
\end{scope}

\begin{scope}[shift={(2.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d31) at (0,0.20) {};
    \node (d32) at (0,0.55) {};
    \node (d33) at (0,1.65) {};
\end{scope}

\begin{scope}[shift={(3.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d41) at (0,0.05) {};
    \node (d42) at (0,1.20) {};
\end{scope}

\begin{scope}[shift={(4.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d51) at (0,0.25) {};
    \node (d52) at (0,0.60) {};
    \node (d53) at (0,1.35) {};
    \node (d54) at (0,1.90) {};
\end{scope}

\begin{scope}[shift={(5.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d61) at (0,0.10) {};
    \node (d62) at (0,0.60) {};
    \node (d63) at (0,1.40) {};
\end{scope}

\begin{scope}[shift={(6.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d71) at (0,0.40) {};
    \node (d72) at (0,0.90) {};
\end{scope}

\begin{scope}[shift={(7.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d81) at (0,0.00) {};
    \node (d82) at (0,0.70) {};
    \node (d83) at (0,1.05) {};
\end{scope}

\begin{scope}[shift={(0.0,-0.5)}]
    \draw[help lines, color=gray!90, dashed] (-0.5, 0.10) grid (7.5, 2.50);
    \draw[-{Stealth[scale=0.9,angle'=45]}, thick] (-0.5,0)--(7.5,0) node[right]{$t$};
\end{scope}
% ============================================================
% Detections over 8 frames
% ============================================================




% ============================================================
% Temporal window & output box & input box
% ============================================================
\draw [line width=2pt, rounded corners=2pt, temporalwindowcolor, dashed] (0.5, -0.4) rectangle (5.5, 2.3);
\draw [line width=2pt, rounded corners=2pt, temporalwindowcolor] (1.5, -0.3) rectangle (6.5, 2.2);

\draw [rounded corners=2pt, top color=red, bottom color=red, opacity=0.3] (3.7, -0.7) rectangle (4.3, 2.6);
\draw [rounded corners=2pt, top color=green, bottom color=green, opacity=0.3] (5.7, -0.7) rectangle (6.3, 2.6);

\node [] at (6.0, -1.0) {Incoming frame};
\node [] at (4.0, 2.9) {Output frame};
% ============================================================
% Temporal window & output box & input box
% ============================================================



% ============================================================
% old solution
% ============================================================
\draw [line width=1.0mm, draw=trajectory1color, dashed]
(d22) -- (d31);

\draw [line width=1.0mm, draw=trajectory2color, dashed]
(d21) -- (d32);
% ============================================================
% old solution
% ============================================================

% ============================================================
% current solution
% ============================================================
\draw [line width=1.0mm, draw=trajectory1color]
(d31) -- (d41)
(d41) -- (d51)
(d51) -- (d61)
(d61) -- (d71);

\draw [line width=1.0mm, draw=trajectory2color]
(d32) -- (d42)
(d42) -- (d53)
(d53) -- (d63)
(d63) -- (d72);

\draw [line width=1.0mm, draw=trajectory3color]
(d33) edge [bend right=15] (d52)
(d52) -- (d62);
% ============================================================
% current solution
% ============================================================




\end{tikzpicture}


==> figures/tracker_model_online.tex <==
%!TEX root = ../egpaper_for_review_suppmat.tex
\begin{tikzpicture}\footnotesize

\definecolor{temporalwindowcolor}{RGB}{90, 90, 90}
\definecolor{outputboxcolor}{RGB}{122, 61, 226}
\definecolor{incomingframeboxcolor}{RGB}{0, 150, 250}


\definecolor{trajectory1color}{RGB}{23, 120, 207}
\definecolor{trajectory2color}{RGB}{222, 16, 17}
\definecolor{trajectory3color}{RGB}{16, 222, 17}

%222, 16, 150

% ============================================================
% Detections over 8 frames
% ============================================================
\begin{scope}[shift={(0.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d11) at (0,0.00) {};
    \node (d12) at (0,0.60) {};
\end{scope}

\begin{scope}[shift={(1.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d21) at (0,0.00) {};
    \node (d22) at (0,0.70) {};
    \node (d23) at (0,1.40) {};
\end{scope}

\begin{scope}[shift={(2.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d31) at (0,0.20) {};
    \node (d32) at (0,0.55) {};
    \node (d33) at (0,1.65) {};
\end{scope}

\begin{scope}[shift={(3.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d41) at (0,0.05) {};
    \node (d42) at (0,1.20) {};
\end{scope}

\begin{scope}[shift={(4.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d51) at (0,0.25) {};
    \node (d52) at (0,0.60) {};
    \node (d53) at (0,1.35) {};
    \node (d54) at (0,1.90) {};
\end{scope}

\begin{scope}[shift={(5.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d61) at (0,0.10) {};
    \node (d62) at (0,0.60) {};
    \node (d63) at (0,1.40) {};
\end{scope}

\begin{scope}[shift={(6.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d71) at (0,0.40) {};
    \node (d72) at (0,0.90) {};
\end{scope}

\begin{scope}[shift={(7.0,0.0)},every node/.style={circle,thick,draw,inner sep=1.5pt}]
    \node (d81) at (0,0.00) {};
    \node (d82) at (0,0.70) {};
    \node (d83) at (0,1.05) {};
\end{scope}

\begin{scope}[shift={(0.0,-0.5)}]
    \draw[help lines, color=gray!90, dashed] (-0.5, 0.10) grid (7.5, 2.50);
    \draw[-{Stealth[scale=0.9,angle'=45]}, thick] (-0.5,0)--(7.5,0) node[right]{$t$};
\end{scope}
% ============================================================
% Detections over 8 frames
% ============================================================




% ============================================================
% Temporal window & output box & input box
% ============================================================
\draw [line width=2pt, rounded corners=2pt, temporalwindowcolor, dashed] (0.5, -0.4) rectangle (5.5, 2.3);
\draw [line width=2pt, rounded corners=2pt, temporalwindowcolor] (1.5, -0.3) rectangle (6.5, 2.2);

\draw [rounded corners=2pt, top color=red, bottom color=green, opacity=0.3] (5.7, -0.7) rectangle (6.3, 2.6);

\node [] at (6.0, -1.0) {Incoming frame};
\node [] at (6.0, 2.9) {Output frame};
% ============================================================
% Temporal window & output box & input box
% ============================================================



% ============================================================
% old solution
% ============================================================
\draw [line width=1.0mm, draw=trajectory1color, dashed]
(d22) -- (d31);

\draw [line width=1.0mm, draw=trajectory2color, dashed]
(d21) -- (d32);
% ============================================================
% old solution
% ============================================================

% ============================================================
% current solution
% ============================================================
\draw [line width=1.0mm, draw=trajectory1color]
(d31) -- (d41)
(d41) -- (d51)
(d51) -- (d61)
(d61) -- (d71);

\draw [line width=1.0mm, draw=trajectory2color]
(d32) -- (d42)
(d42) -- (d53)
(d53) -- (d63)
(d63) -- (d72);

\draw [line width=1.0mm, draw=trajectory3color]
(d33) edge [bend right=15] (d52)
(d52) -- (d62);
% ============================================================
% current solution
% ============================================================




\end{tikzpicture}

